Statistics of the MLE and Approximate Upper and Lower Bounds - Part 1: Application to TOA Estimation

In nonlinear deterministic parameter estimation, the maximum likelihood estimator (MLE) is unable to attain the Cramer-Rao lower bound at low and medium signal-to-noise ratios (SNR) due the threshold and ambiguity phenomena. In order to evaluate the achieved mean-squared-error (MSE) at those SNR levels, we propose new MSE approximations (MSEA) and an approximate upper bound by using the method of interval estimation (MIE). The mean and the distribution of the MLE are approximated as well. The MIE consists in splitting the a priori domain of the unknown parameter into intervals and computing the statistics of the estimator in each interval. Also, we derive an approximate lower bound (ALB) based on the Taylor series expansion of noise and an ALB family by employing the binary detection principle. The accurateness of the proposed MSEAs and the tightness of the derived approximate bounds are validated by considering the example of time-of-arrival estimation.

==> mybiblio.tex <==
\begin{thebibliography}{1}
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% Threshold effect %%%%%%%%%%%%%%%%%%%%%%%%%%
%
\bibitem{ziv}
J. Ziv, and M. Zakai, ``Some lower bounds on signal parameter estimation," 
IEEE Transactions on Information Theory, vol. 15, no. 3, pp. 386--391, May 1969.
%
\bibitem{part2}
A. Mallat, et al. ``Statistics of the MLE and approximated upper and lower bounds -- Part 2: Threshold computation and optimal signal design for minimum achievable MSE," Submitted to ... .
%
%\bibitem{ziv}
%J. Ziv and M. Zakai, 
%``Some lower bounds on signal parameter estimation," 
%IEEE Trans. Inf. Theory, vol. 15, no. 3, pp. 386--391, May 1969.
%
\bibitem{seidman2}
L. P. Seidman, 
``Performance limitations and error calculations for parameter estimation," 
Proceedings of the IEEE, vol. 58, no. 5, pp. 644--652, May 1970.
%
\bibitem{bellini}
S. Bellini, and G. Tartara, 
``Bounds on Error in Signal Parameter Estimation," 
IEEE Trans. Commun., vol. 22, no. 3, pp. 340--342, March 1974.
%
\bibitem{chow}
Siu-Kay Chow, and P. Schultheiss, 
``Delay estimation using narrow-band processes,"
IEEE Transactions on Acoustics, Speech and Signal Processing, vol. 29, no. 3, pp. 478--484, June 1981.
%
\bibitem{weiss1}
A. Weiss, E. Weinstein, 
``Fundamental limitations in passive time delay estimation--Part I: Narrow-band systems," 
IEEE Transactions on Acoustics, Speech and Signal Processing, vol. 31, no. 2, pp. 472--486, April 1983.
%
\bibitem{weiss2}
E. Weinstein, A. Weiss, 
``Fundamental limitations in passive time-delay estimation--Part II: Wide-band systems," 
IEEE Transactions on Acoustics, Speech and Signal Processing, vol. 32, no. 5, pp. 1064--1078, October 1984.
%
\bibitem{zeira1}
A. Zeira, and P. M. Schultheiss, 
``Realizable lower bounds for time delay estimation,"
IEEE Transactions on Signal Processing, vol. 41, no. 11, pp. 3102--3113, November 1993.
%
\bibitem{zeira2}
A. Zeira, and P. M. Schultheiss, 
``Realizable Lower Bounds for Time Delay Estimation: Part 2-Threshold Phenomena,"
IEEE Transactions on Signal Processing, vol. 42, no. 5, pp. 1001--1007, May 1994.
%
\bibitem{sadler1}
B. M. Sadler, and R. J. Kozick,
``A Survey of Time Delay Estimation Performance Bounds," 
Fourth IEEE Workshop on Sensor Array and Multichannel Processing, pp. 282--288, July 2006.
%
\bibitem{sadler2}
B. M. Sadler, L. Huang; Z. Xu, 
``Ziv-Zakai Time Delay Estimation Bound for Ultra-Wideband Signals," 
IEEE International Conference on Acoustics, Speech and Signal Processing (ICASSP 2007), vol.3, pp. 549--552, April 2007.
%
%%%%%%%%%%%%%%%%%%%%%%%%%% Lower and upper bounds %%%%%%%%%%%%%%%%%%%%%%%%
%
\bibitem{renaux}
A. Renaux, 
``Contribution \`a l'analyse des performances d'estimation en traitement statistique du signal," 
Ph.D. dissertation, Laboratory SATIE, ENS CACHAN, Cachan, 2006.
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%% Deterministic bounds %%%%%%%%%%%%%%%%%%%%%%%%
%
\bibitem{kay}
S. Kay, 
``Fundamentals of Statistical Signal Processing Estimation Theory," 
Prentice-Hall, 1993.% pp 53-56
%
\bibitem{barankin}
E. W. Barankin, 
``Locally best unbiased estimators," 
Ann. Math. Statist., vol. 20, pp. 477--501, Dec. 1949.
% 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% ZZLB %%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
%\bibitem{ziv}
%J. Ziv and M. Zakai, 
%``Some lower bounds on signal parameter estimation," 
%IEEE Trans. Inf. Theory, vol. 15, no. 3, pp. 386-ñ391, May 1969.
%
%\bibitem{bellini}
%S. Bellini, and G. Tartara, 
%``Bounds on Error in Signal Parameter Estimation," 
%IEEE Trans. Commun., vol. 22, no. 3, pp. 340--342, March 1974.
% 
\bibitem{chazan}
D. Chazan, M. Zakai, and J. Ziv, 
``Improved lower bounds on signal parameter estimation," 
IEEE Trans. Inf. Theory, vol. 21, no.1, pp. 90--93, Jan. 1975.
%
\bibitem{weinstein}
E. Weinstein, 
``Relations between Belini-Tartara, Chazan-Zakai-Ziv, and Wax-Ziv lower bounds," 
IEEE Trans. Inform. Theory, vol. 34, no. 2, pp. 342--343, March 1988.
% 
\bibitem{bell}
K. L. Bell, Y. Steinberg, Y. Ephraim, and H. L. Van Trees, 
``Extended Ziv-Zakai lower bound for vector parameter estimation," 
IEEE Trans. Inf. Theory, vol. 43, no. 2, pp. 624--637, Mar 1997.
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%% Upper bound %%%%%%%%%%%%%%%%%%%%%%%%%%
%
\bibitem{seidman1}
L. Seidman, 
``An upper bound on average estimation error in nonlinear systems," 
IEEE Transactions on Information Theory, vol. 14, no. 2, pp. 243--250, March 1968.
%
%%%%%%%%%%%%%%%%%%%% Barabkin bound and applications %%%%%%%%%%%%%%%%%%%%%
%
%\bibitem{barankin}
%E. W. Barankin, 
%``Locally best unbiased estimators," 
%Ann. Math. Statist., vol. 20, pp. 477--501, Dec. 1949.
% 
\bibitem{mcaulay1}
R. J. McAulay and L. P. Seidman, 
``A useful form of the Barankin bound and its application to PPM threshold analysis," 
IEEE Trans. Informat. Theory, vol. 15, no.2, pp. 273--279, Mar. 1969.
% 
\bibitem{mcaulay2}
R. J. McAulay and E. Hofstetter, 
``Barankin Bounds on Parameter Estimation," 
IEEE Trans. Informat. Theory, vol. 17, no. 6, pp. 669--676, Nov. 1971.
% 
\bibitem{swerling}
P. Swerling, 
``Parameter Estimation for Waveforms in Additive Gaussian Noise,"
Journal of the Society for Industrial and Applied Mathematics, vol. 7, no. 2, pp. 152--166, June 1959.
% 
%\bibitem{seidman2}
%L. P. Seidman, 
%``Performance limitations and error calculations for parameter estimation," 
%Proceedings of the IEEE , vol. 58, no. 5, pp. 644--652, May 1970.
%
%\bibitem{chow}
%Siu-Kay Chow, and P. Schultheiss, 
%``Delay estimation using narrow-band processes,"
%IEEE Transactions on Acoustics, Speech and Signal Processing, vol. 29, no. 3, pp. 478--484, June 1981.
% A. Zeira, and P. M. Schultheiss, ``Realizable lower bounds for time delay estimation,"
%
%\bibitem{zeira1}
%A. Zeira, and P. M. Schultheiss, 
%``Realizable lower bounds for time delay estimation,"
%IEEE Transactions on Signal Processing, vol. 41, no. 11, pp. 3102--3113, November 1993.
% 
%\bibitem{zeira2}
%A. Zeira, and P. M. Schultheiss, 
%``Realizable Lower Bounds for Time Delay Estimation: Part 2-Threshold Phenomena,"
%IEEE Transactions on Signal Processing, vol. 42, no. 5, pp. 1001--1007, May 1994.
% 
\bibitem{knockaert}
L. Knockaert, 
``The Barankin bound and threshold behavior in frequency estimation,"
IEEE Transactions on Signal Processing, vol. 45, no. 9, pp. 2398--2401, September 1997.
%
%%%%%%%%%%%%%%%%%%%%%%%%%% Applications to the ZZLB %%%%%%%%%%%%%%%%%%%%%%
% 
\bibitem{seidman3}
L. P. Seidman, 
``The performance of a PPM/PM hybrid modulation system," 
IEEE Transactions on Communication Technology, vol. 18, no. 5, pp. 697--698, October 1970.
% 
\bibitem{dardari1}
D. Dardari, C.-C. Chong, and M. Z. Win, 
``Improved Lower Bounds on Time-of-Arrival Estimation Error in Realistic UWB Channels," 
The 2006 IEEE 2006 International Conference on Ultra-Wideband, pp. 531--537, Sept. 2006.
% 
%\bibitem{sadler1}
%B. M. Sadler, and R. J. Kozick,
%``A Survey of Time Delay Estimation Performance Bounds," 
%Fourth IEEE Workshop on Sensor Array and Multichannel Processing, pp. 282--288, July 2006.
% 
%\bibitem{sadler2}
%B.M. Sadler, L. Huang; Z. Xu, 
%``Ziv-Zakai Time Delay Estimation Bound for Ultra-Wideband Signals," 
%IEEE International Conference on Acoustics, Speech and Signal Processing (ICASSP 2007), vol.3, pp. 549--552, April 2007.
%
\bibitem{sadler3}
L. Huang, Z. Xu, and B. M. Sadler, 
``Simplified ziv-zakai time delay estimation bound for ultra-wideband signals," 
Workshop on Short-Range Ultra-Wideband Radio Systems, April 2006.
% 
\bibitem{sadler4}
R. J. Kozick, B. M. Sadler, 
``Bounds and algorithms for time delay estimation on parallel, flat fading channels," 
IEEE International Conference on Acoustics, Speech and Signal Processing (ICASSP 2008), pp. 2413--2416, March 2008.
% 
\bibitem{sinan}
Zafer Sahinoglu, Sinan Gezici and Ismail Guvenc, 
``Ultra-wideband Positioning Systems: Theoretical Limits, Ranging Algorithms, and Protocols," 
New York: Cambridge University Press, 2008.
% 
\bibitem{dardari2}
D. Dardari, C.-C. Chong, and M. Z. Win, 
``Threshold-based time-of-arrival estimators in UWB dense multipath channels," 
IEEE Trans. Commun., vol. 56, no. 8, pp. 1366--1378, Aug. 2008.
% 
\bibitem{dardari3}
D. Dardari, A. Conti, U. Ferner, A. Giorgetti, and M.Z. Win, 
``Ranging With Ultrawide Bandwidth Signals in Multipath Environments," 
Proceedings of the IEEE, vol. 97, no. 2, pp. 404--426, Feb. 2009.
% 
\bibitem{dardari4}
D. Dardari, and M. Z. Win, 
``Ziv-Zakai bound on time-of-arrival estimation with statistical channel knowledge at the receiver," 
Proceedings of the IEEE International Conference on Ultra-Wideband (ICUWB 2009), pp. 624--629, September 2009.
%
%%%%%%%%%%%% Subdomain Wozencraft method and applications %%%%%%%%%%%%%%%
%
\bibitem{wozencraft}
J. M. Wozencraft, and I. M. Jacobs, 
``Principles of Communication Engineering," 
New York: Wiley, 1965.
% 
\bibitem{mcaulay3}
R. McAulay, and D. Sakrison, 
``A PPM/PM Hybrid Modulation System," 
IEEE Trans. Commun. Technol., vol. 17, no. 4, pp. 458--469, Aug. 1969.
% 
\bibitem{seidman4}
L. P. Seidman, 
``A class of signals for analog telemetry over a coherent channel," 
IEEE Trans. Aerospace and Electronic Systems, pp. 645--653, July 1969.
% 
%\bibitem{seidman2}
%L. P. Seidman, 
%``Performance limitations and error calculations for parameter estimation," 
%Proceedings of the IEEE , vol. 58, no. 5, pp. 644--652, May 1970.
%
\bibitem{rife}
D. Rife, and R. Boorstyn, 
``Single tone parameter estimation from discrete-time observations," 
IEEE Transactions on Information Theory, vol. 20, no. 5, pp. 591--598, September 1974.
% 
\bibitem{athley}
F. Athley, 
``Threshold region performance of maximum likelihood direction of arrival estimators," 
IEEE Transactions on Signal Processing, vol. 53, no. 4, pp. 1359--1373, April 2005.
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% 
\bibitem{mallat1}
A. Mallat, J. Louveaux, and L. Vandendorpe, 
``UWB Based Positioning in Multipath Channels: CRBs for AOA and for Hybrid TOA-AOA Based Methods," 
IEEE International Conf. on Commun. (ICC 07), pp. 5775--5780, June 2007.
% 
\bibitem{fcc}
Federal Communications Commission, 
``Revision of Part 15 of the Commissionís Rules Regarding Ultra-Wideband Transmission Systems," 
FCC 02--48, April 2002.
% 
\bibitem{ec1}
Electronic Communications Committee, 
``Commission decision of 21/II/2007 on allowing the use of the radio spectrum for equipment 
using ultra-wideband technology in a harmonised manner in the Community," 21 Feb. 2007. 
% 
\bibitem{ec2}
Electronic Communications Committee, 
``Final Report from CEPT in response to EC Mandates on the harmonized introduction of radio 
applications based on ultra-wideband (UWB) technology," 12 March 2007.
%
\bibitem{molisch}
A. F. Molisch, et all,
``A comprehensive model for ultrawideband propagation channels," 
IEEE Global Telecommunications Conf. (GLOBECOM 05), vol. 6, Dec. 2005.
%
\bibitem{mallat2}
A. Mallat, C. Oestges, and L. Vandendorpe,
``CRBs for UWB Multipath Channel Estimation: Impact of the Overlapping Between the MPCs on MPC Gain and TOA Estimation," 
IEEE International Conf. on Commun. (ICC 09), pp. 1--6, June 2009.
%
\bibitem{mallat3}
A. Mallat, et all, 
``Testbed for IR-UWB based ranging and positioning: Experimental performance and comparison to CRLBs," 
5th IEEE International Symposium on Wireless Pervasive Computing (ISWPC 2010), pp. 163--168, May 2010 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% 
\bibitem{jacobson}
H. I. Jacobson, ``The Maximum Variance of Restricted Unimodal Distributions," 
The Annals of Mathematical Statistics, vol. 40, no. 5, pp. 1746--1752, 
Oct. 1969.
% 
\bibitem{dharmadhikari}
S. W. Dharmadhikari, and K. Joag-Dev, ``Upper bounds for the variances of 
certain random variables," 
Communications in Statistics - Theory and Methods, vol. 18, no. 9, 
pp. 3235--3247, 1989.
%
%\bibitem{urkowitz}
%H. Urkowitz, ``Signal Theory and Random Processes," Artech House, 1983.
% 
%\bibitem{poor}
%H. V. Poor, ``An Introduction to Signal Detection and Estimation," Springer, 
%1988.
% 
%\bibitem{benedetto}
%M-G. Di Benedetto, et all, ``Understanding Ultra Wide Band Radio Fundamentals," 
%Prentice Hall PTR, 2004. % pp. 429-431 pp. 191
% 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\bibitem{genz1}
A. Genz, 
``Numerical Computation of Multivariate Normal Probabilities," 
Journal of Computational and Graphical Statistics, vol. 1, no. 2, pp. 141--149, June 1992.
% 42
\bibitem{genz2}
H. Niederreiter, 
``On a Number-Theoretical Integration Method," 
Aequationes Mathematicae, vol. 8, no. 3, pp. 304--11, October 1972.
% 
\bibitem{genz3}
R. Cranley, and T.N.L. Patterson, 
``Randomization of Number Theoretic Methods for Multiple Integration," 
SIAM Journal on Numerical Analysis, vol. 13, no. 6, pp. 904--914, December 1976.
% 
\bibitem{genz4}
D. Nuyens, and R. Cools, 
``Fast Component-by-Component Construction, a 
Reprise for Different Kernels," H. Niederreiter and D. Talay editors, Monte-Carlo and Quasi-Monte Carlo Methods 2004, pp. 371--385, June 2004.
% 
\bibitem{Marsaglia1964}
G. Marsaglia, 
``Ratios of Normal Variables and Ratios of Sums of Uniform Variables," 
Journal of the American Statistical Association, vol. 60, no. 309, pp. 193--204, March 1965.
% 
\bibitem{Marsaglia2006}
G. Marsaglia, 
``Ratios of Normal Variables," 
Journal of Statistical Software, vol. 16, Issue 4, May 2006.
% 
\bibitem{Hinkley}
D. V. HINKLEY, 
``On the ratio of two correlated normal random variable," 
Biometrika, vol. 56, no. 3, pp. 635--639, Dec. 1969.
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% 
\bibitem{Cinlar}
E. Cinlar, ``Introduction to Stochastic Process," Englewood Cliffs, NJ: 
Prentice Hall, 1975.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\end{thebibliography}
